A Simple Sublinear-Time Algorithm for Counting Arbitrary Subgraphs via Edge Sampling

In the subgraph counting problem, we are given a input graph $G(V, E)$ and a target graph $H$; the goal is to estimate the number of occurrences of $H$ in $G$. Our focus here is on designing sublinear-time algorithms for approximately counting occurrences of $H$ in $G$ in the setting where the algorithm is given query access to $G$. This problem has been studied in several recent papers which primarily focused on specific families of graphs $H$ such as triangles, cliques, and stars. However, not much is known about approximate counting of arbitrary graphs $H$. This is in sharp contrast to the closely related subgraph enumeration problem that has received significant attention in the database community as the database join problem. The AGM bound shows that the maximum number of occurrences of any arbitrary subgraph $H$ in a graph $G$ with $m$ edges is $O(m^{\rho(H)})$, where $\rho(H)$ is the fractional edge-cover of $H$, and enumeration algorithms with matching runtime are known for any $H$. We bridge this gap between subgraph counting and subgraph enumeration by designing a sublinear-time algorithm that can estimate the number of any arbitrary subgraph $H$ in $G$, denoted by $\#H$, to within a $(1\pm \epsilon)$-approximation w.h.p. in $O(\frac{m^{\rho(H)}}{\#H}) \cdot poly(\log{n},1/\epsilon)$ time. Our algorithm is allowed the standard set of queries for general graphs, namely degree queries, pair queries and neighbor queries, plus an additional edge-sample query that returns an edge chosen uniformly at random. The performance of our algorithm matches those of Eden et.al. [FOCS 2015, STOC 2018] for counting triangles and cliques and extend them to all choices of subgraph $H$ under the additional assumption of edge-sample queries. We further show that our algorithm works for the more general database join size estimation problem and prove a matching lower bound for this problem.

==> app-edge-cover.tex <==

\section{Missing Details from Section~\ref{sec:edge-cover}}\label{app:edge-cover}

\subsection{Proof of Lemma~\ref{lem:subgraph-decomposition}}\label{app:subgraph-decomposition}

We now provide a self-contained proof of Lemma~\ref{lem:subgraph-decomposition} (restated below) for completeness. 

\begin{lemma*}[Lemma~\ref{lem:subgraph-decomposition} in Section~\ref{sec:edge-cover}]
	Any subgraph $H$ admits an optimal fractional edge-cover $x^*$ such that the support of $x^*$, denoted by $\supp{x^*}$, is a collection of vertex-disjoint
	odd cycles and star graphs, and, 
	\begin{enumerate}
		\item for every odd cycle $C \in \supp{x^*}$, $x^*_e = 1/2$ for all $e \in C$;
		\item for every edge $e \in \supp{x^*}$ that does \emph{not} belong to any odd cycle,  $x_e = 1$. 
	\end{enumerate}
\end{lemma*}

To prove Lemma~\ref{lem:subgraph-decomposition}, we first state a basic property of LP~(\ref{lp:ec}). 
\begin{proposition}\label{prop:half-integrality-ec}
	LP~(\ref{lp:ec}) admits a half-integral optimum solution $x^* \in \set{0,\frac{1}{2},1}^{\card{E(H)}}$.  Moreover, if $H$ is bipartite, then LP~(\ref{lp:ec}) admits an integral optimum solution. 
\end{proposition}
\begin{proof}
	Suppose first that $H$ is bipartite and $x \in [0,1]^{\card{E(H)}}$ is some optimal solution of LP~(\ref{lp:ec}). We perform a simple cycle-canceling on $x$ to make it integral. In particular, let 
	$e_1,\ldots,e_{2k}$ for some integer $k \geq 2$ be a cycle in the support of $x$ (as $H$ is bipartite length of this cycle is necessarily even). We can alternatively increase the value on one edge and decrease the value
	on the next one by the same amount and continue along the cycle until the value on an edge drops to zero. This operation clearly preserves the feasibility as well as the value of the solution. By doing this, we can cancel all cycles in the support of $x$ 
	without changing the value of LP or violating the feasibility. At this point, support of $x$ is a forest and can be turned into an integral solution using a standard deterministic rounding in a bottom up approach from the leaf-nodes of the forest (see the proof 
	of Lemma~\ref{lem:subgraph-decomposition} for more details on this standard procedure).  
	
	Now suppose $H$ is a non-bipartite graph. Create the following bipartite graph $H'$ where $V(H')$ consists of two copies of vertices in $H$, i.e., for any vertex $a \in V(H)$, there are two copies, say, $a^L$ and $a^R$ in $V(H')$. 
	Moreover, for any edge $e:=(a,b) \in E(H)$ there are two edges $e_1:=(a^L,b^R)$ and $e_2:=(a^R,b^L)$ in $E(H')$. It is easy to see that any edge cover $y$ of $H'$ can be translated to an edge cover $x$ of $H$ by
	setting $x_e = \frac{y_{e_1}+y_{e_2}}{2}$. As by the first part, $H'$ admits an integral optimum solution, we immediately have that $H$ admits a half-integral optimum solution.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:subgraph-decomposition}]
	Let $x^*$ be a half-integral optimum solution for the graph $H$ that is guaranteed to exist by Proposition~\ref{prop:half-integrality-ec}. Let $C$ be any cycle (odd or even length) in $\supp{x^*}$. For any edge $e \in C$, 
	$x^*_e = 1/2$ as otherwise by decreasing $x^*_e$ from $1$ to $1/2$ (recall that $x^*$ is half-integral and $x^*_e \neq 0$), we can reduce the optimal solution without violating the feasibility. Moreover, if 
	$C$ is of even length, then we can perform a standard cycle canceling (by adding and subtracting $1/2$ to the value of $x^*$ on the alternate edges of $C$)
	and remove the cycle. Now suppose $C$ is of odd length; we argue that for each vertex $a$ in $C$, the only edges in $\supp{x^*}$ that are incident on $a$ are the edges in $C$.	
	
	Suppose by contradiction that there exists an edge $e$ with $x^*_e \geq 1/2$ which is incident on a vertex $a$ in an odd cycle $C$ (in $\supp{x^*}$). Perform a cycle canceling as follows: subtract $1/2$ 
	from every other edge starting from an edge incident to $a$ and add $1/2$ to every other edge \emph{plus} the edge $e$. As $C$ is an odd cycle, the total number of addition and subtractions are equal and hence 
	does not change the value of $x^*$. It is also easy to verify that the new $x^*$ is still feasible as $x^*_e \geq 1$ now and hence $a$ is covered still. 
	Thus, by repeatedly applying the above argument, we can change $x^*$ so that $\supp{x^*}$ consists of a vertex-disjoint union of odd cycles (with $x^*_e = 1/2$) and forests. We now turn the forests into a collection of 
	starts using a simple deterministic rounding. 
	
	For each tree $T$ in this forest, we root the tree arbitrarily at some degree one vertex.  Any edge $e$ incident on leaf-nodes of this tree clearly has $x^*_e = 1$.  Let $f$ be a parent edge $e$ and $z$ be
	a parent of $f$ (if these edges do not exist, $e$ belongs to a cycle and we are already done). Let $x^*_z \leftarrow x^*_z + x^*_f$ and $x^*_f \leftarrow 0$. This preserves both the value of $x^*$ and its feasibility, and further partition this 
	tree into a forest and a star. By repeatedly applying this argument, we can decompose every forest into a collection of stars, finalizing the proof of  Lemma~\ref{lem:subgraph-decomposition}. 
\end{proof}








